Fair Representation Clustering with Several Protected Classes

We study the problem of fair $k$-median where each cluster is required to have a fair representation of individuals from different groups. In the fair representation $k$-median problem, we are given a set of points $X$ in a metric space. Each point $x\in X$ belongs to one of $\ell$ groups. Further, we are given fair representation parameters $\alpha_j$ and $\beta_j$ for each group $j\in [\ell]$. We say that a $k$-clustering $C_1, \cdots, C_k$ fairly represents all groups if the number of points from group $j$ in cluster $C_i$ is between $\alpha_j |C_i|$ and $\beta_j |C_i|$ for every $j\in[\ell]$ and $i\in [k]$. The goal is to find a set $\mathcal{C}$ of $k$ centers and an assignment $\phi: X\rightarrow \mathcal{C}$ such that the clustering defined by $(\mathcal{C}, \phi)$ fairly represents all groups and minimizes the $\ell_1$-objective $\sum_{x\in X} d(x, \phi(x))$. We present an $O(\log k)$-approximation algorithm that runs in time $n^{O(\ell)}$. Note that the known algorithms for the problem either (i) violate the fairness constraints by an additive term or (ii) run in time that is exponential in both $k$ and $\ell$. We also consider an important special case of the problem where $\alpha_j = \beta_j = \frac{f_j}{f}$ and $f_j, f \in \mathbb{N}$ for all $j\in [\ell]$. For this special case, we present an $O(\log k)$-approximation algorithm that runs in $(kf)^{O(\ell)}\log n + poly(n)$ time.

==> notation.tex <==
%\usepackage{algorithm}
%\usepackage{algorithmic}

%\usepackage{amsfonts,amsmath,amssymb,mathtools,xfrac}
\usepackage{xspace}
%\usepackage[margin=1in]{geometry}
%\usepackage{natbib}
\usepackage{hyperref}
\usepackage{tikz}
\hypersetup{%
   breaklinks,%
   colorlinks=true,%
   linkcolor=black,%
   urlcolor=black,%
   citecolor=[rgb]{0,0,0.45}
}
\usepackage{xcolor}
\usepackage{enumitem}
% for the table results
\usepackage[utf8]{inputenc}
\usepackage{booktabs}

\usepackage[amsmath,thmmarks]{ntheorem}%
\theoremstyle{plain}%
\newtheorem{theorem}{Theorem}[section]

\newtheorem{result}{Result}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim} 
\newtheorem{fact}[theorem]{Fact}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{invariant}[theorem]{Invariant}
\newtheorem{question}[theorem]{Question}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{openproblem}[theorem]{Open Problem}
\newtheorem{definition}[theorem]{Definition}


%\theoremheaderfont{\bf} \theorembodyfont{\upshape}%
\newtheorem{remark}[theorem]{Remark}%
\newtheorem*{remark:unnumbered}[theorem]{Remark}%
\newtheorem*{remarks}[theorem]{Remarks}%
\newtheorem{example}[theorem]{Example}



% Proof environment

\theoremheaderfont{\em}%
\theorembodyfont{\upshape}%
\theoremstyle{nonumberplain}%
\theoremseparator{}%
\theoremsymbol{\myqedsymbol}%
\newtheorem{proof}{Proof:}%

\newcommand{\myqedsymbol}{$\square$}

\newtheorem{proofof}{Proof of\!}%





\newcommand{\eps}{\varepsilon}%
\def\bar{\overline}
\def\floor#1{\lfloor {#1} \rfloor}
\def\ceil#1{\lceil {#1} \rceil}
\def\script#1{\mathcal{#1}}
\def\etal{\text{et al.}\xspace}
\def\Union{\bigcup}
\def\sep{\;|\;}
\def\card#1{|#1|}
\def\set#1{\{#1\}}
\def\E{\mathbf{E}}
\def\Var{\mathbf{Var}}

\newcommand{\argmax}{\mathrm{argmax}{}\xspace}
\newcommand{\argmin}{\mathrm{argmin}{}\xspace}

\def\wrt{\text{w.r.t.}\xspace}

\newcommand{\polylog}{\mathop{\mathrm{polylog}}}%
\newcommand{\poly}{\mathop{\mathrm{poly}}}%

\def\whp{\text{w.h.p.}}
\newcommand{\tldO}{\widetilde{O}}%
\newcommand{\tldOmega}{\widetilde{\Omega}}%
\newcommand{\tldTheta}{\widetilde{\Theta}}%


\def\sA{\script{A}}
\def\sB{\script{B}}
\def\sC{\script{C}}
\def\sD{\script{D}}
\def\sF{\script{F}}
\def\sG{\script{G}}
\def\sI{\script{I}}
\def\sL{\script{L}}
\def\sK{\script{K}}
\def\sM{\script{M}}
\def\sN{\script{N}}
\def\sO{\script{O}}
\def\sQ{\script{Q}}
\def\sS{\script{S}}
\def\sT{\script{T}}
\def\sU{\script{U}}
\def\sV{\script{V}}
\def\sY{\script{Y}}
\def\sW{\script{W}}
\def\sX{\script{X}}
\def\sZ{\script{Z}}

\def\NP{\ensuremath{\mathrm{\mathbf{NP}}}}
\def\opt{\textsc{OPT}}

\newcommand\faircost{{\operatorname{fair-cost}}}


